An End-to-End Learning-based Cost Estimator

Cost and cardinality estimation is vital to query optimizer, which can guide the plan selection. However traditional empirical cost and cardinality estimation techniques cannot provide high-quality estimation, because they cannot capture the correlation between multiple columns. Recently the database community shows that the learning-based cardinality estimation is better than the empirical methods. However, existing learning-based methods have several limitations. Firstly, they can only estimate the cardinality, but cannot estimate the cost. Secondly, convolutional neural network (CNN) with average pooling is hard to represent complicated structures, e.g., complex predicates, and the model is hard to be generalized. To address these challenges, we propose an effective end-to-end learning-based cost estimation framework based on a tree-structured model, which can estimate both cost and cardinality simultaneously. To the best of our knowledge, this is the first end-to-end cost estimator based on deep learning. We propose effective feature extraction and encoding techniques, which consider both queries and physical operations in feature extraction. We embed these features into our tree-structured model. We propose an effective method to encode string values, which can improve the generalization ability for predicate matching. As it is prohibitively expensive to enumerate all string values, we design a patten-based method, which selects patterns to cover string values and utilizes the patterns to embed string values. We conducted experiments on real-world datasets and experimental results showed that our method outperformed baselines.

==> src/improvement.tex <==
\section{Improvement}
\subsection{Tree-LSTM}
Instead of encoding the plan tree and the predicates tree into 1-dimension vectors, we can denote each node as a LSTM Cell, the parent cell take the sum of children as input and output its result. This method has two advantages, it can represent the structure of the data directly and it can reduce the overhead by avoiding assigning LSTM cell for assistant null node.
\subsection{MDP-style Training}
For the tree recursive neural network model, we actually learn the representations of sub-plans step by step. When we learn a query, we can set the loss as an holistic error of all steps of the plan (Representation Cell in this paper). Specifically, we stack one output layer upon each Cell and get the estimation on cost and cardinality, all these estimation errors combined together can be the loss. In another words, we train the query in a Markov Decision Process manner where transform probability and actions are all determined.
